ROMEVA: Geometry-Preserving Vocabulary Expansion for Roman Urdu Language Models

Multilingual Language Models like mBERT are widely used for low-resource NLP, yet their adaptation to morphologically inconsistent languages such as Roman Urdu remains underexplored. Roman Urdu spelling variation causes severe sub-word fragmentation, averaging 1.50 sub-words per token. We propose \textit{ROMEVA} (Roman Urdu Embedding-preserving Vocabulary Adaptation), which combines sub-word-average initialization and a PCA-guided anchor loss to stabilize embeddings during vocabulary expansion. Using a 36,130-comment Roman Urdu corpus, we add 500 highly fragmented tokens to mBERT and compare naive fine-tuning, sub-word-aware fine-tuning, and \textit{ROMEVA}. While \textit{ROMEVA} most effectively preserves the pretrained embedding space, naive fine-tuning achieves the strongest downstream sentiment classification performance. These findings reveal a disconnect between embedding stability and downstream performance, suggesting that stronger adaptation may be preferable to strict embedding preservation in morphologically inconsistent languages.

==> extra.tex <==
%\subsection{Models and Optimization}
\subsection{Tokenization for Low-Resource and Informal Text}

Recent NLP systems commonly use subword tokenization methods such as Byte Pair Encoding (BPE) \cite{sennrich-etal-2016-neural} and SentencePiece \cite{kudo-richardson-2018-sentencepiece}. Both methods struggle with informal romanized languages where spelling variation is high. In Roman Urdu, a single word can appear in multiple forms (e.g., "kya", "kia", "kiya"), leading to excessive subword fragmentation and weak semantic consistency.

This study builds upon Multilingual BERT (mBERT) \cite{devlin-etal-2019-bert}, a pretrained model trained on 104 languages, it is primarily trained on formal Wikipedia-style text and does not explicitly account for Roman Urdu. As a result, Roman Urdu inputs often exhibit high subword fragmentation.

\subsection{Domain-Adaptive Pretraining and Vocabulary Expansion}

Domain-Adaptive Pretraining (DAPT) \cite{gururangan-etal-2020-dont} assumes that the existing tokenizer remains suitable for the target domain. This assumption is often violated in Roman Urdu due to high spelling variation and vocabulary mismatch.

Vocabulary expansion extends pretrained models by adding new tokens to the embedding space and continuing training on domain-specific data. While this improves coverage, it can also introduce instability in pretrained representations due to updates affecting both newly added and existing embeddings.

\subsection{Continual Learning and Embedding Stability}

Continual learning focuses on preserving previously learned knowledge while adapting to new tasks. Elastic Weight Consolidation (EWC) \cite{kirkpatrick2017overcoming} addresses catastrophic forgetting by penalizing changes to important parameters using Fisher information.

The geometric structure of embedding spaces has also been widely studied. \cite{mu-viswanath-2018-all} show that meaningful semantic information is concentrated in the top principal components of embedding spaces. Similarly, \cite{ethayarajh-2019-contextual} demonstrates that contextualized representations exhibit structured and constrained geometric properties. These findings suggest that preserving key semantic directions may help maintain representation stability during adaptation.

\subsubsection{Dynamic Tokenization}
Recent work has begun exploring adaptive tokenization. \cite{wang2025pit} propose PIT (Personalized Item Tokenizer), which jointly adapts tokenization and model representations in recommendation systems. This demonstrates the potential of making tokenization a learnable component rather than a fixed preprocessing step. However, prior work has not specifically examined tokenization-induced embedding drift in Roman Urdu or its impact on vocabulary expansion settings.

\subsection{Evaluation}

\subsubsection{Embedding Drift Measurement}

\cite{lazaridou2021mind} analyzes representational shifts in language models trained on different time periods, while \cite{kulkarni2015statistically} proposes statistical methods to detect semantic change at the word level. These studies show that embedding drift is measurable using geometric metrics such as cosine similarity and distributional distance. Accordingly, L2 drift and cosine similarity are appropriate measures for quantifying embedding drift during adaptation.

% A key methodological distinction in this work is the separation between global and corpus-specific drift. While averaging drift over the entire vocabulary may dilute the observed effect, focusing only on tokens appearing in Roman Urdu text provides a more accurate estimate of domain-specific representation change.

\subsubsection{Downstream Sentiment Evaluation}

Roman Urdu sentiment analysis and code-mixed South Asian sentiment analysis remain relatively under-resourced compared to native Urdu NLP. Most existing datasets are based on Nastaliq script, which differs significantly from Roman Urdu in vocabulary and orthography.

In this work, downstream evaluation is conducted on the RUWV-NSR dataset \citep{soomro2024dataset}, a five-class Roman Urdu sentiment dataset containing 28,090 samples. 

% The use of five-class classification provides a more fine-grained evaluation compared to binary sentiment settings, where class distinctions are often easier to separate.

\subsubsection{Tokenization Analysis as a Diagnostic Tool}

Fragmentation ratio, defined as the average number of subword tokens produced per word, has been used in prior work as an informal indicator of vocabulary mismatch. In this study, fragmentation analysis is used as a diagnostic tool for identifying out-of-vocabulary candidates and motivating vocabulary expansion in low-resource Roman Urdu settings.

==> images/prompt.tex <==


\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{p{0.97\columnwidth}}
\toprule
\rowcolor{lightgray}
\textbf{Prompt} \\
\midrule
\rowcolor{lightergray}
\textbf{Task:} \\
I want to perform data augmentation because of class imbalance, and this class has very few examples. I want to generate 30 more examples of the class \textit{{class\_name}}. \\
\midrule
\rowcolor{lightgray}
\textbf{Class Definition:} \\
\textit{{definition of class}} \\
\midrule
\rowcolor{lightergray}
\textbf{Instructions:} \\
I have given you 15 examples below from the dataset for your understanding. Study the examples and follow their structuring and other characteristics to generate new examples that align with this definition in the context of the slogans in political debates dataset. \\
\midrule
\rowcolor{lightgray}
\textbf{Examples (15 total):} \\
\textbf{Example 1} \\
\textbf{Text:} \textit{{sample from training data 1}} \\
\textbf{Fallacy Type:} \textit{{class\_name}} \\[1ex]

\textbf{Example 2} \\
\textbf{Text:} \textit{{sample from training data 2}} \\
\textbf{Fallacy Type:} \textit{{class\_name}} \\[1ex]

% ... repeat for remaining examples ...

\bottomrule
\end{tabular}
\end{adjustbox}

==> tbs/tb0.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\toprule
\citep{ct1965} & \verb|\citep| & \verb|\cite| \\
\citealp{ct1965} & \verb|\citealp| & no equivalent \\
\citet{ct1965} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{ct1965} & \verb|\citeyearpar| & \verb|\shortcite| \\
\citeposs{ct1965} & \verb|\citeposs| & no equivalent \\
\citep[FFT;][]{ct1965} &  \verb|\citep[FFT;][]| & no equivalent\\
\bottomrule
\end{tabular}
\end{adjustbox}


==> tbs/tb1.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ll}
\toprule
\textbf{Fallacy Type} & \textbf{Description} \\
\midrule
Ad Hominem & Personal attacks instead of addressing the argument. \\
Appeal to Authority & Unjustified reliance on authority as evidence. \\
Appeal to Emotion & Persuasion by emotional manipulation rather than logic. \\
False Cause & Incorrect causal attributions without sufficient evidence. \\
Slogan & Use of catchphrases lacking argumentative substance. \\
Slippery Slope & Assuming one action leads to extreme outcomes without basis. \\
\bottomrule
\end{tabular}
\end{adjustbox}

==> tbs/tb2.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ll | ll}
\toprule
\textbf{Text-only} & \textbf{M-F1} & \textbf{Audio-only} & \textbf{M-F1} \\
\midrule
RoBERTaB\footref{fn0} & 0.5441 & WhisperS & \textbf{0.3168} \\
RoBERTaL\footref{fn1} & 0.4439 & WhisperT & 0.1800 \\
DistilBERTB\footref{fn2} & 0.4369 & WhisperB w/ FE & 0.1275 \\
BERTB\footref{fn3} & 0.3939 & Wav2Vec2.0 & 0.1262 \\
ElectraB & 0.3945 & Whisper+aug. & 0.1260 \\
DeBERTaB & 0.4856 & Wav2Vec+aug. & 0.2400 \\
RoBERTaS & 0.4418 & MFCC+2D-CNN & 0.1281 \\
RoBERTaB (aug. data) & \textbf{0.5786} & MFCC+GaussianNB & 0.1764 \\
DistilRoBERTaB (aug. data) & 0.4418 & MFCC+Logistic Regression & 0.1622 \\
& & MFCC+SGDClassifier & 0.1622 \\
\bottomrule
\end{tabular}
\end{adjustbox}




==> tbs/tb3.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|l|l|}
\hline
\textbf{File/Folder}        & \textbf{Description} \\ \hline
\verb|main.tex|             & Main content file; includes sections and calls to other files. \\ \hline
\verb|preamble.tex|         & Contains all \LaTeX{} packages and user-defined commands for cleaner main file. \\ \hline
\verb|img/|                 & Folder for all figures in PDF format (no JPG or PNG). \\ \hline
\quad\verb|arch.pdf|        & Example of a figure stored in the \verb|img/| folder. \\ \hline
\verb|tbs/|                 & Folder to store table code files separately for modularity. \\ \hline
\quad\verb|tb0.tex|         & Example of a table stored in the \verb|tbs/| folder. \\ \hline
\verb|references.bib|       & BibTeX file containing all references for citation. \\ \hline
\end{tabular}
\end{adjustbox}
